Causal Inference With Selectively Deconfounded Data

Given only data generated by a standard confounding graph with unobserved confounder, the Average Treatment Effect (ATE) is not identifiable. To estimate the ATE, a practitioner must then either (a) collect deconfounded data;(b) run a clinical trial; or (c) elucidate further properties of the causal graph that might render the ATE identifiable. In this paper, we consider the benefit of incorporating a large confounded observational dataset (confounder unobserved) alongside a small deconfounded observational dataset (confounder revealed) when estimating the ATE. Our theoretical results suggest that the inclusion of confounded data can significantly reduce the quantity of deconfounded data required to estimate the ATE to within a desired accuracy level. Moreover, in some cases -- say, genetics -- we could imagine retrospectively selecting samples to deconfound. We demonstrate that by actively selecting these samples based upon the (already observed) treatment and outcome, we can reduce sample complexity further. Our theoretical and empirical results establish that the worst-case relative performance of our approach (vs. a natural benchmark) is bounded while our best-case gains are unbounded. Finally, we demonstrate the benefits of selective deconfounding using a large real-world dataset related to genetic mutation in cancer.

==> sections/lower_bound.tex <==
%\section{Lower Bound}


%In Proposition~\ref{prop:hardness}, we constructed such a $\bf q$ pairs by setting one of the entries of the $\bf q$. Next, assuming that each entry of $\bf q$ is bounded away from zero, i.e., $q_{yt}\in[\eta, 1-\eta]$ for some small positive constants $\eta>0$, we show that 




==> sections/old files/finite_cache.tex <==
In Section~\ref{sec:methods}, we showed that 
\emph{given an infinite amount of confounded data}
and tasked with selecting examples to deconfound
(based on the observed values of $T$ and $Y$,
OWSP outperforms the {\em natural} sampling policy 
both in the worst case and in expectation 
with respect to a uniform distribution 
over underlying parameters $\bf a, q$.

In this section, we extend our analysis to the case
where we only have access to a finite amount of confounded data. 
In particular, we start with no confounded data and a budget of size $B$. 
In this setting, we must first decide the value of $n$---the 
amount of confounded data that we wish to acquire.
% Let $n$ denote the amount of confounded data 
% available.
% that we decided to acquire, and then 
These $n$ confounded data provide us with an \emph{estimate} 
of the \textbf{confounded distribution}, $\hat{P}_{Y,T}(\cdot,\cdot)$.
After acquiring the confounded data, to estimate the \textbf{conditional distributions}, $\hat{P}_{Z|Y,T}(\cdot|y,t)$, 
we need to either reveal the value of $z$ for some chosen confounded data 
or sample tuples of deconfounded data, $(y,t,z)$. 
In the first part of this section, we focus on the former. 
In the second part of this section, we will discuss the latter.
% 
% In this setting, we must allocate a fixed budget $B$ among the following activities:
% (i) acquiring more confounded data;
% and (ii) 
% After acquiring the confounded data, we now need to
% deconfound (reveal $z$) for some data with known $(y, t)$. 
Here, we fix some cost  $c_c$ for obtaining one extra confounded data point 
and a (possibly different) cost $c_z$ to reveal the value of a confounder $z$.
Given our underlying motivation, we are principally interested 
in the case where obtaining confounded data is cheaper 
than deconfounding, i.e., $c_c < c_z$. 
% In addition, we are interested in the case where we have a total budget of $B$ to spend on both acquiring confounded data and deconfounding $z$.


% In this setting, the confounded can only provide us with 
% an estimate of the \textbf{confounded distribution}, $\hat{P}_{Y,T}(\cdot,\cdot)$.
% Thus, we may examples naturally, we gain information 
% Selectively deconfounding, in this case, means to select $m$ confounded data to reveal their value for the unobserved confounder, $Z$.
% % 
% 
% In practice, selectively deconfounding can be achieved by following up with current patients with smart bottles to track their treatment adherence levels.$\hat{P}_{Z|Y,T}(\cdot|y,t)$
% This procedure only provides an estimated \textbf{conditional distributions}, $\hat{P}_{Z|Y,T}(\cdot|y,t)$. 
% 
% In other words, selectively deconfounding cannot be used to update $\hat{P}_{Y,T}(\cdot,\cdot)$. Thus, to update $\hat{P}_{Y,T}(\cdot,\cdot)$, we need to collect additional data. 
% When the cost of collecting additional confounded data is low,
% relative to the cost of deconfounding,
% the benefits of selective deconfounding become more pronounced. 

Given the setup above, in this section, 
we first address the following question:
when we selectively deconfound a finite dataset, 
when (in terms of the observed data and known cost structure)
% trade-off between acquiring more confounded data $n$
% and deconfounding more data, $m_{sd}$.
is it preferable to spend our budget to acquire additional confounded data 
vs. to selectively-deconfound additional examples.
With $x_{yt}$ defined in Section~\ref{sec:methods}, We first derive a theorem analogous to Theorems \ref{thm_m0}-\ref{thm_m2} (the proof of the theorem is included in Appendix~\ref{proof:thm5}):
% the following theorem characterizes the trade-offs mentioned above. 
\begin{theorem}\label{thm5}
% Given budget $B$,
After acquiring $n$ confounded data, and $m$ deconfounded examples, with the fraction of examples selected from each among the $4$ groups (defined by their $T$, $Y$ values) given by $\mathbf{x}$
$P\left(\left|\text{ATE}-\widehat{\text{ATE}}\right|\geq\epsilon\right)\leq \delta$ is satisfied when
\begin{align*}
&\exp\Bigg(-2\left(\frac{\epsilon}{12}\right)^2\min\Bigg(
{\frac{(p_7+p_3)^2}{\frac{1}{x_{11}m}+\frac{q_4^2}{n}}}, 
{\frac{(p_8+p_4)^2}{\frac{1}{x_{11}m}+\frac{(1-q_4)^2}{n}}}, 
\\&
{\frac{(p_7+p_3)^2}{\frac{1}{x_{01}m}+\frac{q_2^2}{n}}},
{\frac{(p_8+p_4)^2}{\frac{1}{x_{01}m}+\frac{(1-q_2)^2}{n}}},
{\frac{(p_5+p_1)^2}{\frac{1}{x_{10}m}+\frac{q_3^2}{n}}}, 
{\frac{(p_6+p_2)^2}{\frac{1}{x_{10}m}+\frac{(1-q_3)^2}{n}}},
\\&
{\frac{(p_5+p_1)^2}{\frac{1}{x_{00}m}+\frac{q_1^2}{n}}},
{\frac{(p_6+p_2)^2}{\frac{1}{x_{00}m}+\frac{(1-q_1)^2}{n}}}\Bigg)\Bigg) \leq
\frac{\delta}{16}.
% \text{ and } c_z m + c_c n \leq B.
\end{align*}
\end{theorem}

Similar to Section~\ref{sec:methods}, our baseline policy is \emph{natural} selection policy. To implement natural, under this setup, is to set $m=n$, that is, we deconfound all confounded data that we acquired. Let $\hat{a_i}$ be our empirical estimate of $a_i$ based on the confounded dataset. 
Then, under the \emph{natural} selection policy, the linear relaxation of the problem gives us $m_{nat} = n_{nat} = \frac{B}{c_c+c_z}$, that is, $P\left(\left|\text{ATE}-\widehat{\text{ATE}}\right|\geq\epsilon\right)\leq \delta$ is satisfied when the amount of samples satisfies
\begin{align*}
& \exp\Bigg(-2(\frac{\epsilon}{12})^2\frac{B}{c_c+c_z}\min\Big(
{\frac{(p_7+p_3)^2}{\frac{1}{\widehat{a_4}}+q_4^2}}, 
{\frac{(p_8+p_4)^2}{\frac{1}{\widehat{a_4}}+(1-q_4)^2}}, 
\\&
{\frac{(p_7+p_3)^2}{\frac{1}{\widehat{a_2}}+q_2^2}},
{\frac{(p_8+p_4)^2}{\frac{1}{\widehat{a_2}}+(1-q_2)^2}},
{\frac{(p_5+p_1)^2}{\frac{1}{\widehat{a_3}}+q_3^2}}, 
{\frac{(p_6+p_2)^2}{\frac{1}{\widehat{a_3}}+(1-q_3)^2}},
\\&
{\frac{(p_5+p_1)^2}{\frac{1}{\widehat{a_1}}+q_1^2}},
{\frac{(p_6+p_2)^2}{\frac{1}{\widehat{a_1}}+(1-q_1)^2}}\Big)\Bigg) \leq
\frac{\delta}{16}.
\end{align*}

There are few reasons why that we would sample more confounded and deconfound less, that is $m<n$. First, it provides a better estimate to $x_{yt}$ under \emph{OWSP}. 
Since $c_c<c_z$, giving up one deconfounded $z$ can give more than one confounded data point. 
We have seen in Section~\ref{sec:methods} that \emph{OWSP} is more efficient in deconfounding than \emph{natural} and \emph{uniform} selection policy. 
Thus sampling more confounded data could potentially make the deconfounding process more efficient.
Second, the $n_{nat}$ confounded data we have might not contain enough data that we can implement \emph{uniform} selection policy or \emph{OWSP}. That is, we might not have enough data of type $(y,t)$ in the confounded data to deconfound. In the analysis below, we first derive the properties for $m$ and $n$ under \emph{uniform} selection policy and \emph{OWSP}. We then analyze the sample complexity associated with these two selection policies.
% In the analysis below, we will first ignore the first the second condition when deriving the properties for $m$ and $n$ under \emph{uniform} selection policy and \emph{OWSP}, that is, we assume that our confounded dataset always contain enough data to deconfound. We will then discuss second condition in detail.

First, under the \emph{uniform} selection policy, we have $x_{yt} = \frac{1}{4} $ $\forall y,t \in \{0,1\}$. However, to adjust for the fact that there might not be enough data to deconfound, we need to choose $x_{yt}=\min (\frac{1}{4}, \frac{\widehat{P_{Y,T}(y,t)}n}{m})$, with $\widehat{P_{Y,T}(y,t)}$ be the same as the ones under \emph{natural} selection policy. Thus, to minimize the estimation error subject to the budget constraint, we need to solve the following optimization problem:
% Now, we are ready to incorporate the budget constraint, that is, the maximum amount of money that we can spend on acquiring additional confounded data and selectively-deconfounding additional examples is $B$. To solve for this budget constraint, we formulate the following optimization problem:
\begin{align*}
\max \limits_{m,n} \min \Big({\frac{(p_7+p_3)^2}{\frac{\max(4,\frac{m}{n\widehat{a_4}})}{m}+\frac{q_4^2}{n}}}, &{\frac{(p_8+p_4)^2}{\frac{\max(4,\frac{m}{n\widehat{a_4}})}{m}+\frac{(1-q_4)^2}{n}}},
\\{\frac{(p_7+p_3)^2}{\frac{\max(4,\frac{m}{n\widehat{a_2}})}{m}+\frac{q_2^2}{n}}},
&{\frac{(p_8+p_4)^2}{\frac{\max(4,\frac{m}{n\widehat{a_2}})}{m}+\frac{(1-q_2)^2}{n}}},
\\
{\frac{(p_5+p_1)^2}{\frac{\max(4,\frac{m}{n\widehat{a_3}})}{m}+\frac{q_3^2}{n}}},
&
{\frac{(p_6+p_2)^2}{\frac{\max(4,\frac{m}{n\widehat{a_3}})}{m}+\frac{(1-q_3)^2}{n}}},
\\
{\frac{(p_5+p_1)^2}{\frac{\max(4,\frac{m}{n\widehat{a_1}})}{m}+\frac{q_1^2}{n}}},
&
{\frac{(p_6+p_2)^2}{\frac{\max(4,\frac{m}{n\widehat{a_1}})}{m}+\frac{(1-q_1)^2}{n}}}\Big)
\\
% \quad\quad
% \end{align*}
% \begin{align*}
\text{s.t.} \quad c_z m + c_c n &\leq B
\\m & \leq n
\\ 
m,n &\in \mathcal{Z}^{+}
\end{align*}
To ease the problem, we will solve for the linear relaxation of the problem, that is,
substituting the constraint, $c_z m + c_c n = B$, into the objective function, we obtain the following:
{
% \footnotesize
\begin{align*}
& \max \limits_{0\leq m\leq \frac{B}{c_c + c_z}} \min \Big(
{\frac{(p_7+p_3)^2}{\frac{\max(4,\frac{c_c m}{\widehat{a_4}(B-c_z m)})}{m}+\frac{c_c q_4^2}{B-c_z m}}},
\\&
{\frac{(p_8+p_4)^2}{\frac{\max(4,\frac{c_c m}{\widehat{a_4}(B-c_z m)})}{m}+\frac{c_c(1-q_4)^2}{B-c_z m}}}, 
{\frac{(p_7+p_3)^2}{\frac{\max(4,\frac{c_c m}{\widehat{a_2}(B-c_z m)})}{m}+\frac{c_c q_2^2}{B-c_z m}}},
\\&
{\frac{(p_8+p_4)^2}{\frac{\max(4,\frac{c_c m}{\widehat{a_2}(B-c_z m)})}{m}+\frac{c_c(1-q_2)^2}{B-c_z m}}},
{\frac{(p_5+p_1)^2}{\frac{\max(4,\frac{c_c m}{\widehat{a_3}(B-c_z m)})}{m}+\frac{c_c q_3^2}{B-c_z m}}}, 
\\&
{\frac{(p_6+p_2)^2}{\frac{\max(4,\frac{c_c m}{\widehat{a_3}(B-c_z m)})}{m}+\frac{c_c(1-q_3)^2}{B-c_z m}}},
{\frac{(p_5+p_1)^2}{\frac{\max(4,\frac{c_c m}{\widehat{a_1}(B-c_z m)})}{m}+\frac{c_c q_1^2}{B-c_z m}}},
\\&
{\frac{(p_6+p_2)^2}{\frac{\max(4,\frac{c_c m}{\widehat{a_1}(B-c_z m)})}{m}+\frac{c_c (1-q_1)^2}{B-c_z m}}}\Big). 
% \geq
% \frac{72\ln (\frac{16}{\delta})}{\epsilon^2},    
\end{align*}
}

Let $g_1(m) = \frac{\max(4,\frac{c_c m}{\widehat{a_4}(B-c_z m)})}{m} + \frac{c_c q_4^2}{B-c_z m}$. That is, if $4\widehat{a_4}<1$, then when $m\in[0, \frac{B}{c_z +  \frac{c_c}{4\widehat{a_4}}}], g_1(m) = h_1(m) = \frac{4}{m} + \frac{c_c q_4^2}{B-c_z m}$, and when $m\in [\frac{B}{c_z +  \frac{c_c}{4\widehat{a_4}}},\frac{B}{c_z+c_c}], g_1(m) = l_1(m) = \frac{c_c/\widehat{a_4}+ c_c q_4^2}{(B-c_z m)}
$; if $4\widehat{a_4}\geq 1$, then $g_1(m) = \frac{4}{m} + \frac{c_c q_4^2}{B-c_z m}$.
We now let $f_1(m) = \frac{(p_7+p_3)^2}{g_1(m)}$. 
We define $g_2(m),...,g_8(m)$ and $f_2(m),...,f_8(m)$  respectively for the second to eighth term above. 

First, we show that $f_i(m)$ is concave on $[0,\frac{B}{c_c+c_z}]$ $\forall i \in [8]$. We will illustrate this using $g_1(m)$. 
We first observe that $g_1(m)$ is a piecewise convex function:
$h''(m)>0$ and $l''(m)>0$ on $[0,\frac{B}{c_c+c_z}]$.
Second,
$l_1(m)$ is monotonically increasing on $[0,\frac{B}{c_c+c_z}]$: $l'(m) = \frac{c_z (c_c/\widehat{a_4}+ c_c q_4^2)}{(B-c_z m)^2}>0$. Third, $h'(m) = \frac{-4}{m^2}+\frac{c_z c_c q_4^2}{(B-c_z m)^2} < l'(m)$, and $h(\frac{B}{c_z +  \frac{c_c}{4\widehat{a_4}}})=l(\frac{B}{c_z +  \frac{c_c}{4\widehat{a_4}}})$. Putting those three observations together, we have $g_1(m)$ is convex on $[0,\frac{B}{c_c+c_z}]$. Thus, $f_i(m)$ is concave on $[0,\frac{B}{c_c+c_z}]$
$\forall i \in [8]$. 
% Thus, $\frac{(p_7+p_3)^2}{f(m)}$ is concave on $[0,\frac{B}{c_c+c_z}]$. 
Since the minimum of concave functions are concave,
we have the following lemma:
% the maximum of the minimum of concave functions is obtained at either one of the intersection points of these concave functions, or one of the maximum of each concave functions:
\begin{lemma}\label{lemma:concave}
Let $f_1(x), ..., f_{n}(x)$ be $n$ single variable concave functions on $x\in \mathcal{X}$, where $n\in \mathcal{Z}^+$, then $\max\min\left(f_1(x), ..., f_{n}(x)\right) = \min\limits_{i\neq j} \left( \max\min(f_i(x), f_j(x)) \right)$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:concave}]
$\leq$: we observe that $ \min(f_1(x), ..., f_n(x)) \leq \min(f_i(x), f_j(x)) $ for all $i, j \in [n]$. Thus, $\max\min(f_1(x), ..., f_n(x)) \leq \max\limits_{i\neq j} \min(f_i(x), f_j(x))$ for all $i, j \in [n]$. Consequently, $\max\min(f_1(x), ..., f_n(x)) \leq \min \limits_{i\neq j}(\max \min(f_i(x), f_j(x)))$.

$\geq$: Without loss of generality, let $\max\min(f_{i^*}(x), f_{j^*}(x))=\min\limits_{i\neq j} \left( \max\min(f_i(x), f_j(x)) \right)$. For the sake of contradiction, assume that $\max\min\left(f_1(x), ..., f_{n}(x)\right) < \max\min(f_{i^*}(x), f_{j^*}(x))$. This implies that there must exists $l$ s.t. $\max\min(f_{i^*}(x), f_{j^*}(x), f_l(x)) < \max\min(f_{i^*}(x), f_{j^*}(x))$. Then, since $f_{i^*},f_{j^*},f_l$ concave, either $\max\min(f_{i^*}(x), f_l(x)))) < \max\min(f_{i^*}(x), f_{j^*}(x))$ or $\max\min(f_{j^*}(x), f_l(x)))) < \max\min(f_{i^*}(x), f_{j^*}(x))$. Either case contradicts to the fact that $\max\min(f_{i^*}(x), f_{j^*}(x))=\min\limits_{i\neq j} \left( \max\min(f_i(x), f_j(x)) \right)$. 
\end{proof}
\begin{lemma}\label{lemma:intersect}
Let $f_i(x)$ and $f_j(x)$ be two concave functions that only intersects at $x^*$. If $(\argmax f_i(x)-x^*)(\argmax f_j(x)-x^*)\geq 0$, then $\max\min(f_i(x),f_j(x)) = \min(\max f_i(x), \max f_j(x))$, else $\max\min(f_i(x),f_j(x)) = f_i(x^*)$.
\end{lemma}
\begin{lemma}\label{lemma:intersect2}
Let $f_i(x)$ and $f_j(x)$ be two concave functions that intersects at $x_1^*$ and $x_2^*$. If $(\argmax f_i(x_i)-x_i^*)(\argmax f_j(x_i)-x_i^*)\geq 0, \forall x_i=\{1,2\}$, then $\max\min(f_i(x),f_j(x)) = \min(\max f_i(x), \max f_j(x))$, else $\max\min(f_i(x),f_j(x)) = \max\left(f_i(x_1^*), f_i(x_2^*)\right)$.
\end{lemma}

Thus, by Lemma~\ref{lemma:concave}, to find the $\max\min (f_1(m),...,f_8(m))$, it suffices to calculate the $\max\min$ of the 28 combination of two functions. Let's first calculate $\max\min (f_1(m), f_2(m))$. By Lemma~\ref{lemma:intersect}, we first need to calculate $\argmax f_1(m), \argmax f_2(m)$, and $m^*$.
% However, by inspecting $\max\min$ terms carefully, we can reduce the number of combinations to 6.

First, $\argmax f_1(m) = \argmin g_1(m) = \argmin h_1(m)$. 
% Case 1: there is enough data to deconfound according to \emph{uniform} selection policy, i.e., the maximum is attained at $4$. In the case, 
Since when $m=0, h_1(m)=\infty,\argmin g_1(m)=\min \left(\frac{B}{c_c+c_z}, \frac{B}{c_z+\frac{c_c}{4\widehat{a_4}}}, h'^{-1}(0)\right)$. To calculate $h'^{-1}(0)$, we need to solve $\frac{4}{m^2} = \frac{c_c c_z q_4^2}{(B-c_zm)^2}$. This is equivalent to $\frac{(B-c_zm)^2}{m^2} = \frac{c_c c_z q_4^2}{4}$. Taking square root on both sides and solving the rest, we have $h'^{-1}(0) = \frac{B}{\frac{q_4\sqrt{c_zc_c}}{2}+c_z}$. Thus, $\argmin g_1(m)=\min \left(\frac{B}{c_c+c_z},\frac{B}{c_z+\frac{c_c}{4\widehat{a_4}}},\frac{B}{c_c\frac{q_4\sqrt{c_z}}{2\sqrt{c_c}}+c_z} \right)$,
and in the last case, $\max f_1(m) = \frac{B(p_7+p_3)^2}{c_c q_4^2 + 4\sqrt{c_c c_z} q_4 + 4c_z} = \frac{B(p_7+p_3)^2}{(\sqrt{c_c}q_4 + 2\sqrt{c_z})^2}$.
% {\color{red} and $n = \frac{B- c_z m}{c_c} = \frac{Bq_4\sqrt{c_c c_z}}{c_c q_4\sqrt{c_c c_z} + 2c_c c_z}$}. 
% Case 2: there is not enough data to deconfound according to \emph{uniform} selection policy, i.e., the maximum is attained at $\frac{c_c m}{\widehat{a_4}(B-c_z m)}$. In this case, we have $g_1'(m)= \frac{\frac{c_c c_z}{\widehat{a_4}} + c_c c_z q_4^2}{(B-c_z m)^2}$. Notice there is no critical point on $[0,\frac{B}{c_c+c_z}]$, thus $\argmax g_1(m)=0$, and $\max g_1(m) = \frac{B(p_7+p_3)^2}{c_c (\frac{1}{\widehat{a_4}}+q_4^2)}$. 

Now, we find the intersection point of $f_1(m),f_2(m)$, i.e., $m_{1,2}^*$. 
Case 1: $4\widehat{a_4}>1$. In this scenario, setting $\frac{(p_7+p_3)^2}{h_1(m)} = \frac{(p_8+p_4)^2}{h_2(m)}$, we have $m_{1,2}^*=\frac{B}{c_c\frac{(p_7+p_3)^2(1-q_4)^2-(p_8+p_4)^2q_4^2}{4(p_8+p_4)^2-4(p_7+p_3)^2}+c_z}$. Notice that $\frac{(p_7+p_3)^2(1-q_4)^2-(p_8+p_4)^2q_4^2}{4(p_8+p_4)^2-4(p_7+p_3)^2} = \frac{(p_7+p_3)^2(1+q_4^2-2q_4)-(p_8+p_4)^2q_4^2}{4(p_8+p_4)^2-4(p_7+p_3)^2} = -\frac{1}{4}\left(q_4^2-\frac{(1-2q_4)}{\frac{(p_8+p_4)^2}{(p_7+p_3)^2}-1}\right)$ 

% Notice that since the fraction in the denominator is always in $(-0.25,0)$, $m^*$ will always be between $[0,\frac{B}{c_c+c_z}]$. 

On the other hand, $\argmax f_1(m) = \min( \frac{B}{c_c+c_z} ,\frac{B}{c_c\frac{q_4\sqrt{c_z}}{2\sqrt{c_c}}+c_z})$ and $\argmax f_2(m) = \min(\frac{B}{c_c+c_z}, \frac{B}{c_c\frac{(1-q_4)\sqrt{c_z}}{2\sqrt{c_c}}+c_z})$. 

Noting that both the fractions in the denominator is always positive, and thus those two points are on the same side of $m^*$. Thus, in this scenario, by Lemma~\ref{lemma:intersect}, the $\max\min (f_1(m),f_2(m)) = \min(\max f_1(m),\max f_2(m))$. {\color{red} $\sqrt{\frac{c_z}{c_c}}$ need to satisfy some condition.}

Case 2: $4\widehat{a_4}\leq 1$.
% there is not enough data to deconfound according to \emph{uniform} selection policy, i.e., the maximum is achieved at $\frac{c_c m}{\widehat{a_4}(B-c_z m)}$. 
In this case, to find $m_{1,2}^*$, in addition to the intersection point in case 1, we also need to check whether $\frac{(p_7+p_3)^2}{l_1(m)}$ and $\frac{(p_8+p_4)^2}{l_2(m)}$, $\frac{(p_7+p_3)^2}{h_1(m)}$ and $\frac{(p_8+p_4)^2}{l_2(m)}$, and $\frac{(p_7+p_3)^2}{l_1(m)}$ and $\frac{(p_8+p_4)^2}{h_2(m)}$ intersect. First, to check whether $\frac{(p_7+p_3)^2}{l_1(m)}$ intersects with $\frac{(p_8+p_4)^2}{l_2(m)}$, we solve $\frac{(p_7+p_3)^2(B-c_z m)}{c_c/\widehat{a_4} +c_c q_4^2}= \frac{(p_8+p_4)^2(B-c_z m)}{c_c/\widehat{a_4}+c_c(1-q_4)^2 }$. One can verify that $f_1(m)$ and $f_2(m)$ either overlap or do not intersect on $[0,\frac{B}{c_c+c_z}]$. Second, to check whether $\frac{(p_7+p_3)^2}{h_1(m)}$ and $\frac{(p_8+p_4)^2}{l_2(m)}$ intersect, we solve $\frac{(p_7+p_3)^2}{\frac{4}{m}+\frac{c_c q_4^2}{B-c_z m}} = \frac{(p_8+p_4)^2(B-c_z m)}{\frac{c_c}{\widehat{a_4}}+c_c(1-q_4)^2}$, and this gives us that $m_{1,2}^* = \frac{B}{c_c\left(\frac{(p_7+p_3)^2}{4(p_8+p_4)^2}(\frac{1}{\widehat{a_4}
}+(1-q_4)^2)-\frac{q_4^2}{4}\right)+c_z} = \frac{B}{-\frac{c_c}{4}\left(q_4^2-\frac{(p_7+p_3)^2}{(p_8+p_4)^2}(\frac{1}{\widehat{a_4}
}+(1-q_4)^2)\right)+c_z} $.

Thus, in this case, we also have $\max\min (f_1(m),f_2(m)) = \min(\max f_1(m),\max f_2(m))$.

Above, we've seen that $\max\min(f_1(m),f_2(m)) = \min(\max f_1(m), \max f_2(m))$. Similarly, this holds for $\max\min(f_3(m), f_4(m)), \max\min(f_5(m), f_6(m))$, and $\max\min(f_7(m),f_8(m)).$ 

Now, let's calculate $\max\min (f_1(m),f_3(m))$. Case 1: there is enough data to deconfound according to \emph{uniform} selection policy in both $f_1(m)$ and $f_3(m)$, i.e., the maximum is achieved at $4$ in both functions. To find $m^*$, we need to solve ${\frac{(p_7+p_3)^2}{\frac{4}{m}+\frac{c_c q_4^2}{B-c_z m}}}= {\frac{(p_7+p_3)^2}{\frac{4}{m}+\frac{c_c q_2^2}{B-c_z m}}}$.
One can check that $f_1(m)$ and $f_2(m)$ either overlap or do not intersect on $[0,\frac{B}{c_c+c_z}]$. Case 2: there is not enough data to deconfound according to \emph{uniform} in both functions, i.e., the maximum is achieved at $\frac{c_c m}{\widehat{a_4}(B-c_z m)}$. Similar to Case 1, one can verify $f_1(m)$ and $f_2(m)$ either overlap or do not intersect on $[0,\frac{B}{c_c+c_z}]$. Case 3: there is enough data to deconfound according to \emph{uniform} in one function but not the other one. WLOG, let the maximum be achieved at $\frac{c_c m}{\widehat{a_4}(B-c_z m)}$ for the first term and $4$ at the second term. Then $m^*=\min(\frac{B}{c_c+c_z}, \frac{B}{c_c(\frac{1}{4\widehat{a_4}}+\frac{q_4^2-q_2^2}{4})+c_z})$. In this case, $\argmax f_1(m) = 0$, and $\argmax f_3(m)= \min(\frac{B}{c_c+c_z}, \frac{B}{c_c\frac{q_2\sqrt{c_z}}{2\sqrt{c_c}}+c_z})$.
Thus, when $\frac{c_z}{c_c}< (\frac{1}{4\widehat{a_4}}+\frac{q_4^2-q_2^2}{4})^2\frac{4}{q_2^2}, \text{ i.e., } \frac{c_z}{c_c}< (\frac{1}{2\widehat{a_4}q_2}+\frac{q_4^2-q_2^2}{2q_2})^2, \max\min(f_1(m),f_3(m)) = \max f_3(m)$, and otherwise, $\max\min(f_1(m),f_3(m)) = f_1(m^*) = f_3(m^*)$.
% $\max\min(f_1(m),f_3(m)) = \min(\frac{B}{c_c+c_z}, \frac{B}{c_c(\frac{1}{4\widehat{a_4}}+\frac{q_4^2-q_2^2}{4})+c_z})$. Similarly, this analysis applies to the rest $\max\min$ pairs except the ones already mentioned above.

Thus, if we always have enough data to 
An immediate observation is that the ratio between the deconfounded $z$ and confounded data, $\frac{m}{n} =\min(1, \frac{\max(2,\sqrt{\widehat{a_4}})}{q_4}\sqrt{\frac{c_c}{c_z}})$, that is, if $\frac{c_c}{c_z} < \frac{q_4^2}{4}$, the percentage of confounded data to deconfound is proportional to $\sqrt{\frac{c_c}{c_z}}$. 

% Now, let $c_d$ be the cost of sampling a new tuple of deconfounded data, $(y, t, z)$, and if we choose to sample a new tuple of data, we can update both the confounded distribution, $\hat{P}_{Y,T}(\cdot,\cdot)$, and the conditional distributions, $\hat{P}_{Z|Y,T}(\cdot|y,t)$. However, if $c_d \geq c_c + c_z$, sampling a new tuple of deconfounded data seems less effective than both acquiring confounded data and deconfounding the value of one confounder. Thus,
% in the second part of this section, we focus on the scenario where we receive a discounted bundle cost when choose to sample a new tuple, that is $c_d < c_z + c_c$. 
% % Notice that under this setup, sampling one  

% % On the other hand, sampling according to {\em natural} selection policy 
% % in the finite confounded data case corresponds 
% % to obtaining a new tuple of data $(y,t,z)$ 
% % that is sampled according to the true distribution $P_{Y,T,Z}$.
% % In practice, sampling according to {\em natural} can be achieved
% % by distributing smart bottles to new patients as well as collect their treatment and outcome data.

% % Sampling according to {\em natural} selection policy will allow us 
% % to update both $\hat{P}_{Y,T}(\cdot,\cdot)$ and $\hat{P}_{Z|Y,T}(\cdot|y,t)$.
% % Notice that if the cost of collecting one additional confounded data 
% % and the cost of obtaining a new tuple of data are the same, 
% % then {\em natural} selection policy will always be preferred 
% % over collecting additional confounded data. 

% Thus, the second question we address in this section is that when estimating ATE according to a finite dataset,
% % given $n$ of confounded data to start with, 
% what is the trade-off
% % 
% % \zack{between acquiring additional confounded data (T,Y) tuples with cost $c_c$
% % and deconfounding data (with cost $c_d$)}
% % 
% between acquiring more confounded data, $n$,
% acquiring new rows of deconfounded data, $m_r$,
% and selectively deconfounding more data, $m-m_r$.
% Similarly, we first derive a theorem analogous to Theorems \ref{thm_m0}-\ref{thm5} (the proof of the theorem is included in Appendix \ref{proof:5_action}):
% % Theorem~\ref{thm:5_action} address characterizes this trade-off.

% % Notice that $m_{sd}$ only consists the value of $Z$, and $m$ consists the value of $(Y,T,Z)$ that is not contained in the confounded data.
% \begin{theorem}\label{thm:5_action}
% When including the option of sampling new tuples of deconfounded data, $P\left(\left|\text{ATE}-\hat{\text{ATE}}\right|\geq\epsilon\right)\leq \delta$ is satisfied when 
% \begin{align*}
% &32\max(
% e^{\frac{-2(m_r+n)(\frac{a_4q_4+a_2q_2}{12}\epsilon)^2}{1+\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}+2\sqrt{\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}}}} ,
% % \\&
% e^{\frac{-2(m_r+n)(\frac{a_4(1-q_4)+a_2(1-q_2)}{12}\epsilon)^2}{1+\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}+2\sqrt{\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}}}},
% \\&
% e^{\frac{-2(m_r+n)(\frac{a_4q_4+a_2q_2}{12}\epsilon)^2}{1+\frac{m_r+n}{x_2(m-m_r)+0.4a_2m_r}+2\sqrt{\frac{m_r+n}{x_2(m-m_r)+0.4a_2m_r}}}},
% % \\&
% e^{\frac{-2(m_r+n)(\frac{a_4(1-q_4)+a_2(1-q_2)}{12}\epsilon)^2}{1+\frac{m_r+n}{x_2(m-m_r)+0.4a_2m_r}+2\sqrt{\frac{m_r+n}{x_2(m-m_r)+0.4a_2m_r}}}},
% \\&
% e^{\frac{-2(m_r+n)(\frac{a_3q_3+a_1q_1}{12}\epsilon)^2}{1+\frac{m_r+n}{x_3(m-m_r)+0.4a_3m_r}+2\sqrt{\frac{m_r+n}{x_3(m-m_r)+0.4a_3m_r}}}},
% % \\&
% e^{\frac{-2(m_r+n)(\frac{a_3(1-q_3)+a_1(1-q_1)}{12}\epsilon)^2}{1+\frac{m_r+n}{x_3(m-m_r)+0.4a_3m_r}+2\sqrt{\frac{m_r+n}{x_3(m-m_r)+0.4a_3m_r}}}}
% \\&
% e^{\frac{-2(m_r+n)(\frac{a_3q_3+a_1q_1}{12}\epsilon)^2}{1+\frac{m_r+n}{x_1(m-m_r)+0.4a_1m_r}+2\sqrt{\frac{m_r+n}{x_1(m-m_r)+0.4a_1m_r}}}},
% % \\&
% e^{\frac{-2(m_r+n)(\frac{a_3(1-q_3)+a_1(1-q_1)}{12}\epsilon)^2}{1+\frac{m_r+n}{x_1(m-m_r)+0.4a_1m_r}+2\sqrt{\frac{m_r+n}{x_1(m-m_r)+0.4a_1m_r}}}}
% )
% % \\&
% % = 32e^{-2(m_r+n)(\frac{\epsilon}{12})^2\min\Big(
% % \frac{(p_7+p_3)^2}{{1+\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}+2\sqrt{\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}}}},
% % (p_8+p_4)^2,
% % (p_5+p_1)^2,
% % (p_6+p_2)^2 \Big)}
% % \\&
% \leq
% \delta,
% \end{align*}
% % and $c_rm_r + c_c n + c_z(m-m_r)\leq B$.
% \end{theorem}


% A quick sanity check on Theorem~\ref{thm5}: when $m\rightarrow \infty$, selectively deconfounding has a positive error because we only have a limited number of confounded samples to estimate the joint distribution of $Y,T$. Whereas the error in Theorem~\ref{thm:5_action} goes to 0, when taking $m_r$ and $m$ both to $\infty$, and this is because acquiring a new row of deconfounded data updates both $P(Y,T)$ and $P(Z|Y,T)$. {\color{red} need to either write a corollary or write more carefully. To do: figure out how to optimize the budget constraint.}


% To add the budget constraint, we formulate the following optimization problem:
% \begin{align*}
% &\max(
% e^{\frac{-2(m_r+n)(\frac{a_4q_4+a_2q_2}{12}\epsilon)^2}{1+\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}+2\sqrt{\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}}}} ,
% % \\&
% e^{\frac{-2(m_r+n)(\frac{a_4(1-q_4)+a_2(1-q_2)}{12}\epsilon)^2}{1+\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}+2\sqrt{\frac{m_r+n}{x_4(m-m_r)+0.4a_4m_r}}}},
% \\&
% e^{\frac{-2(m_r+n)(\frac{a_4q_4+a_2q_2}{12}\epsilon)^2}{1+\frac{m_r+n}{x_2(m-m_r)+0.4a_2m_r}+2\sqrt{\frac{m_r+n}{x_2(m-m_r)+0.4a_2m_r}}}},
% % \\&
% e^{\frac{-2(m_r+n)(\frac{a_4(1-q_4)+a_2(1-q_2)}{12}\epsilon)^2}{1+\frac{m_r+n}{x_2(m-m_r)+0.4a_2m_r}+2\sqrt{\frac{m_r+n}{x_2(m-m_r)+0.4a_2m_r}}}},
% \\&
% e^{\frac{-2(m_r+n)(\frac{a_3q_3+a_1q_1}{12}\epsilon)^2}{1+\frac{m_r+n}{x_3(m-m_r)+0.4a_3m_r}+2\sqrt{\frac{m_r+n}{x_3(m-m_r)+0.4a_3m_r}}}},
% % \\&
% e^{\frac{-2(m_r+n)(\frac{a_3(1-q_3)+a_1(1-q_1)}{12}\epsilon)^2}{1+\frac{m_r+n}{x_3(m-m_r)+0.4a_3m_r}+2\sqrt{\frac{m_r+n}{x_3(m-m_r)+0.4a_3m_r}}}}
% \\&
% e^{\frac{-2(m_r+n)(\frac{a_3q_3+a_1q_1}{12}\epsilon)^2}{1+\frac{m_r+n}{x_1(m-m_r)+0.4a_1m_r}+2\sqrt{\frac{m_r+n}{x_1(m-m_r)+0.4a_1m_r}}}},
% % \\&
% e^{\frac{-2(m_r+n)(\frac{a_3(1-q_3)+a_1(1-q_1)}{12}\epsilon)^2}{1+\frac{m_r+n}{x_1(m-m_r)+0.4a_1m_r}+2\sqrt{\frac{m_r+n}{x_1(m-m_r)+0.4a_1m_r}}}}
% )
% \end{align*}
% \begin{align*}
%     \text{s.t.} \quad c_rm_r + c_c n + c_z(m-m_r)&\leq B
%     \\
%     m_r, m, n &\in \mathcal{Z}^{+}
% \end{align*}

% % In the first two parts of the paper, we established the benefits of including infinite amount of confounded data (alongside with deconfounded data).
% We have seen in Section~\ref{sec:methods} OWSP outperforms {\em natural} sampling policy in both worst-case and in expectation over uniform distribution over the parameters $\bf a, q$ when there is an infinite amount of confounded data.
% In this section, we explore the case where a finite amount of confounded data is available, with the number of confounded data $n<\infty$. Those $n$ confounded data provides us an estimated \textbf{confounded distribution}, $\hat{P}_{Y,T}(\cdot,\cdot)$.

% Selectively deconfounding, in this case, means to select $m$ confounded data to reveal their value for the unobserved confounder, $Z$. In practice, selectively deconfounding can be achieved by following up with current patients with smart bottles to track their treatment adherence levels.
% This procedure only provides an estimated \textbf{conditional distributions}, $\hat{P}_{Z|Y,T}(\cdot|y,t)$. In other words, selectively deconfounding cannot be used to update $\hat{P}_{Y,T}(\cdot,\cdot)$. Thus, to update $\hat{P}_{Y,T}(\cdot,\cdot)$, we need to collect additional confounded data. When the cost of collecting additional confounded data is relatively low, selectively deconfounding becomes an attractive method. Thus, in the first part of the section, we answer the question that when selectively deconfound a finite dataset, what is the optimal ratio of the amount of confounded data, $n$, and confounded entry that we deconfound, $m_{sd}$, assuming the cost of revealing one confounder and collect one addition confounded data are the same.


% On the other hand, sampling according to {\em natural} selection policy in the finite confounded data case corresponds to obtaining a new tuple of data $(y,t,z)$ that is sampled according to the true distribution $P_{Y,T,Z}$.
% In practice, sampling according to {\em natural} can be achieved by distributing smart bottles to new patients as well as collect their treatment and outcome data.
% Sampling according to {\em natural} selection policy will allow us to update both $\hat{P}_{Y,T}(\cdot,\cdot)$ and $\hat{P}_{Z|Y,T}(\cdot|y,t)$.
% Notice that if the cost of collecting one additional confounded data and the cost of obtaining a new tuple of data are the same, then {\em natural} selection policy will always be preferred over collecting additional confounded data. 
% Thus, in the second part of the section, we answer the question that given a fixed amount of confounded data, $n$, what is the trade-off between selectively deconfounding the confounded data, and sampling more deconfounded data $m$ according to {\em natural}, 
% % and obtaining more confounded data,
% assuming the cost of selectively deconfound one data is the same as the cost of obtaining a new data tuple $(y,t,z)$.
% % Notice that $m_{sd}$ only consists the value of $Z$, and $m$ consists the value of $(Y,T,Z)$ that is not contained in the confounded data.



% \begin{theorem}[Sample complexity for 2 independent r.v.s with 2 independent sampling processes]\label{thm3}
% Let $X_1,..., X_n$ and $Y_1, ..., Y_m$ be two sequences of Bernoulli random variables independently drawn from distribution $p_1$ and $p_2$, respectively. Let $S_X= \sum \limits_{i=1}^n X_i, S_Y =\sum \limits_{i=1}^m Y_i$. Then, 
% % $P\Big(S_X S_Y - E[S_X]E[S_Y]\geq nmt \Big)\leq e^{\frac{-2t^2}{\frac{1}{m}+\frac{p_2^2}{n}}}$. By symmetry, we have
% $P\Big(\Big|S_X S_Y - E[S_X]E[S_Y]\Big|\geq nmt\Big)\leq 2\exp\left(\frac{-2t^2}{\frac{1}{m}+\frac{p_2^2}{n}}\right)$.
% \end{theorem}

% \begin{theorem}[Sample complexity for 3 random variables with dependent sampling process]\label{thm4} Let $A_1, ..., A_{m+n}$ be a sequence of random variables drawn independently from binomial($a$); similarly, let $P_1,...,P_{m}$ drawn independently from binomial($p_1$), and $Q_1,..., Q_{m}$ drawn independently from binomial($p_2$). Furthermore, $a=p_1+p_2, A_{N+i}=P_i+Q_i$, $P_iQ_i=0, \forall i$. Let $S_X=\sum \limits_{i=1}^n A_i$, $S_P=\sum \limits_{i=1}^{m} P_i, S_Q=\sum \limits_{i=1}^{m} Q_i$; as a result $\sum \limits_{i=1}^{m+n} A_i=S_X+S_P+S_Q$; then $P\Big(\Big|\frac{S_X+S_P+S_Q}{m+n}\frac{S_P}{S_P+S_Q}-a(\frac{p_1}{p_1+p_2})\Big|\geq t\Big) 
% \leq 
% 4\exp\left(-\frac{2t^2}{\frac{1}{m+n}+\frac{1}{m}+2\sqrt{\frac{1}{m(m+n)}}}\right)$.

% \end{theorem}

% With $x_{yt}$ defined in section~\ref{sec:methods}, the following theorem characterizes the trade-offs mentioned above. 

% \begin{theorem}\label{thm5}
% Given $n$ confounded samples, when selectively deconfounding, the amount of samples required to satisfy $P\left(\left|\text{ATE}-\hat{\text{ATE}}\right|\geq\epsilon\right)\leq \delta$ when
% \begin{align*}
% & \exp\Bigg(-2(\frac{\epsilon}{12})^2\min\Big({\frac{(p_7+p_3)^2}{\frac{1}{x_{11}m}+\frac{q_4^2}{n}}}, {\frac{(p_8+p_4)^2}{\frac{1}{x_{11}m}+\frac{(1-q_4)^2}{n}}}, 
% {\frac{(p_7+p_3)^2}{\frac{1}{x_{01}m}+\frac{q_2^2}{n}}},
% {\frac{(p_8+p_4)^2}{\frac{1}{x_{01}m}+\frac{(1-q_2)^2}{n}}},
% {\frac{(p_5+p_1)^2}{\frac{1}{x_{10}m}+\frac{q_3^2}{n}}}, 
% \\&
% {\frac{(p_6+p_2)^2}{\frac{1}{x_{10}m}+\frac{(1-q_3)^2}{n}}},
% {\frac{(p_5+p_1)^2}{\frac{1}{x_{00}m}+\frac{q_1^2}{n}}},
% {\frac{(p_6+p_2)^2}{\frac{1}{x_{00}m}+\frac{(1-q_1)^2}{n}}}\Big)\Bigg) \leq
% \frac{\delta}{16}.
% \end{align*}
% When sample according to {\em natural} selection policy, $P\left(\left|\text{ATE}-\hat{\text{ATE}}\right|\geq\epsilon\right)\leq \delta$ when 
% $$\exp\left(-\frac{2(\frac{\epsilon}{12})^2}{\frac{1}{m+n}+\frac{1}{m}+2\sqrt{\frac{1}{m(m+n)}}}\min\Big(
% (p_7+p_3)^2,
% (p_8+p_4)^2,
% (p_5+p_1)^2,
% (p_6+p_2)^2 \Big)\right)
% \leq
% \frac{\delta}{32}.$$
% \end{theorem}


==> sections/old files/theoretical.tex <==

%In this section, we provide bounds for the sample size such that $P(|\hat{\mathrm{ATE}}-\mathrm{ATE}|\geq\epsilon)\leq \delta$. The proofs of the theorems can be found in Appendix~\ref{app_proofs}

% \begin{theorem}\label{thm_m0}
% Without using any observational data, 
% $P(|\hat{\mathrm{ATE}}-\mathrm{ATE}|\geq \epsilon)<\delta$ 
% is satisfied if the number of samples
% $m \geq  \frac{18\ln(\frac{16}{\delta})}{\epsilon^2} \max\Big( \frac{1}{(p_3+p_7)^2}, \frac{1}{(p_4+p_8)^2},\frac{1}{(p_1+p_5)^2},\frac{1}{(p_2+p_6)^2} \Big).$
% \end{theorem}


% \begin{theorem}\label{thm_m1}
% When incorporating (infinite) observational data via Method 1, 
% $P(|\hat{\mathrm{ATE}}-\mathrm{ATE}|\geq \epsilon)<\delta$ 
% is satisfied if the number of samples 
% $m \geq  \frac{18\ln(\frac{8}{\delta})}{\epsilon^2} \max\Big( \frac{1}{(p_3+p_7)^2},\frac{1}{(p_4+p_8)^2},\frac{1}{(p_1+p_5)^2},\frac{1}{(p_2+p_6)^2} \Big).$
% \end{theorem}

% \begin{theorem}\label{thm_m2}
% When incorporating (infinite) confounded data, 
% $P(|\hat{\mathrm{ATE}}-\mathrm{ATE}|\geq \epsilon)<\delta$ 

% \begin{itemize}
%     \item if $(x_1, x_2, x_3, x_4)=(a_1, a_2, a_3, a_4)$, i.e., sample according to natural selection policy, then $m_{natural} \geq  \frac{18\ln(\frac{8}{\delta})}{\epsilon^2} \max \Big( \frac{a_2+a_4}{\min((p_3+p_7)^2,(p_4+p_8)^2)},\frac{a_1+a_3}{\min((p_1+p_5)^2,(p_2+p_6)^2)}\Big);$
%     \item if $(x_1, x_2, x_3, x_4)=(1/4,1/4,1/4,1/4)$, i.e., sample according to natural selection policy, then $m_{uniform} \geq  \frac{18\ln(\frac{8}{\delta})}{\epsilon^2} \max \Big( \frac{4 (a_2^2+a_4^2)}{\min((p_3+p_7)^2,(p_4+p_8)^2)},\frac{4 (a_1^2+a_3^2)}{\min((p_1+p_5)^2,(p_2+p_6)^2)}\Big);$
%     \item if $(x_1, x_2, x_3, x_4)=(\frac{a_1}{2(a_1+a_3)},\frac{a_2}{2(a_2+a_4)},\frac{a_3}{2(a_1+a_3)},\frac{a_4}{2(a_2+a_4)})$, i.e., sample according to outcome weighted sampling policy, then $m_{OWSP} \geq  \frac{18\ln(\frac{8}{\delta})}{\epsilon^2} \max \Big( \frac{2(a_2+a_4)^2}{\min((p_3+p_7)^2,(p_4+p_8)^2)},\frac{2(a_1+a_3)^2}{\min((p_1+p_5)^2,(p_2+p_6)^2)}\Big).$
% \end{itemize}

% \end{theorem}
% \begin{remark}
% Sampling according to the ratio always allocates half of the samples to $T=0$ 
% and half of the samples to $T=1$. 
% Furthermore, if we assume the mean of $q_i=\frac{1}{2}$ $\forall i$ (this corresponds to no confounding), 
% then setting $q_i=\frac{1}{2}$ $\forall i$, we have that 
% the number of samples needed in sampling according to ratio is independent of $\mathbf{a}$.
% \end{remark}

% Theorem~\ref{thm_m0}--\ref{thm_m2} suggest that in the case of one uncontrolled confounder, 
% incorporating observational data provides a constant improvement. 
% Our Theorem~\ref{thm_m2} also suggests that the sampling according to ratio dominates uniform sampling 
% in terms of the concentration inequality since $4a_2^2+4a_4^2-2(a_2+a_4)^2=2(a_2-a_4)^2\geq 0$. 
 

% On the other hand, Figure~\ref{fig:agg}--\ref{examples} show that sampling according to the ratio and sampling uniformly dominates sampling according to distribution in expectation of $\mathbf{q}$ when $\mathbf{a}$ is fixed. This leads to the corollary~\ref{cor}. The proof can be found in Appendix~\ref{app_proofs}

% \begin{cor}\label{cor}
% Let $m_{\text{distr}}$ and $m_{\text{ratio}}$ be the lower bounds on the number of samples needed when sampling from distribution and ratio to achieve an estimation error less than $\delta$, respectively. Then,
% $\max \limits_{\mathbf{a}}\frac{m_{\text{ratio}}}{m_{\text{distr}}}\leq 2$ when ${m_{\text{distr}}}\leq {m_{\text{ratio}}}$, and  $ \max \limits_{\mathbf{a}}\frac{m_{\text{distr}}}{m_{\text{ratio}}}\to \infty$ when ${m_{\text{distr}}}\geq {m_{\text{ratio}}}$.
% \end{cor}


% \begin{remark}
% Corollary~\ref{cor} provides an intuitive explanation of why sampling according to ratio on average outperforms sampling from distribution. However, as we will see in the next section, this concentration bound is not tight.
% \end{remark}


==> sections/online.tex <==

\begin{figure*}[!ht]
    \centering
    \begin{subfigure}
    \centering
    \includegraphics[width=0.28\textwidth]{figure/online_4line.pdf}
    \end{subfigure}
    \begin{subfigure}
    \centering
    \includegraphics[width=0.34\textwidth]{figure/online_Scatter_2online150_1000.pdf}
    \end{subfigure}
    \begin{subfigure}
    \centering
    \includegraphics[width=0.34\textwidth]{figure/online_Scatter_owsp_online2_150_1000.pdf}
    \end{subfigure}
    \vspace{-5mm}
    \caption{Performance of online policies (Greedy and 2-Step Lookahead) vs. offline policies (NSP and OWSP), assuming infinite confounded data. Left: averaged over 1,300 distributions, each consisting of $4$ replications. Middle and Right:  $50$ distributions, each averaged over 1,000 replications.}
    \label{fig:online}
\end{figure*}

% Next, to motive our follow-up work on online deconfounding, we show that by carefully selecting samples online, we can further reduce the absolute absolute error by a large margin. 

So far, we have established the benefits 
of using confounded data (alongside deconfounded data) 
in the {\em offline} setting, i.e. where the
%Next, we established the benefits of strategically choosing
%what 
fraction of our deconfounded data allocated 
to each group (as defined by the values of $Y$ and $T$) must be specified upfront.
% Note that in the previous analysis, these fractions were
% fixed a priori as a function of the (known) distribution $P_{Y,T}$. 
%However, as noted in Section~\ref{sec:methods}, 
% This upfront restriction meant that none of our sampling policies could 
%our best offline sampling policy---OWSP---
Note that offline policies
cannot utilize any information about $q_{yt}^z$. 
% Thus, 
We conclude by introducing an {\em online} setting
where we can choose which group to sample from 
sequentially (over $m$ periods) and adaptively,
incorporating information from all previous steps. 
For notational convenience, we will focus on the case 
where the confounder is binary, i.e., $Z\in\{0,1\}$, and denote $q_{yt} = P_{Z=1|Y,T}$.
% (y,t)$.
%of selective deconfounding. 
% s a function of the previous observations under the
% assumption that we access to an infinite amount of confounded data.
%
% Intuitively, after each observation, we update our estimates for each $\hat{q}_{yt}^z$, we then simulate the next data arrival from the current estimated $\hat{q}_{yt}^z$, and choose which group ($yt$) to sample from next, to move the furthermost away from the previous estimated ATE.
%
%Intuitively, the gap between offline and online policies should be substantial since, after each observation, 
%we can update our estimate for each $\hat{q}_{yt}^z$
%(both its value and uncertainty),
%and choose the group (${yt}$) from which to sample  %next,
%to most rapidly decrease our uncertainty over the ATE.
% Let $i$ denote the current period (ranging from 1 to $m$) of the online problem. 

We will again assume that we have infinitely many confounded samples. %Recall that when we have an infinite amount of confounded data, 
Recall that this implies $a_{yt}$ is known for all $y,t$, and thus, 
the only parameters we need to estimate are $q_{yt}$, for all $y,t$.
% 
At each period, we can represent the {\em state} as a tuple $$(n_{00},n_{01},n_{10},n_{11},\hat{q}_{00},\hat{q}_{01},\hat{q}_{10},\hat{q}_{11}),$$ 
where $n_{yt}$ is the number of previous periods where group $yt$ was chosen, 
and $\hat{q}_{yt}$ is the proportion of these periods for which $Z = 1$ was observed
(initialized to be $\frac{1}{2}$ if $n_{yt}=0$). 
The $\hat{q}_{yt}$'s coincide with our running estimates of the $q_{yt}$'s, 
and we will continue to estimate the $\ATE$ by plugging these estimates into \eqref{equ:def}.
%
An online policy is then a mapping from the state to the four groups. 
% As before, our estimator $\hat{q}_{yt}^i$ for any $q_{yt}$ is the maximum likelihood estimator (initialized to be $\frac{1}{2}$ if no observations have occurred), and our estimator $\widehat{\ATE}^i$ for the $\ATE$ is gotten by plugging these values into \eqref{equ:def}. Finally, abusing notation slightly, we let $\widehat{\ATE}(X_{yt}^i = z)$ denote the estimated $\ATE$ in the next period if were to observe value $z$ from group $(y,t)$.
%\textbf{Online Sample Selection Policy }
Here, we propose two online policies for selective deconfounding. %Due to space requirements, we give short descriptions here, and provide more complete descriptions in the Appendix. 
% Since the ATE is a nonlinear function of the parameters $q_{yt}$, 
% at each step, 
% % to estimate the uncertainty over ATE, 
% to translate the uncertainty over $q_{yt}$ to the uncertainty over ATE,
% we hold everything else constant and perturb the one of the estimated $\hat{q}_{yt}$s.

% by adding one more sample from the group $yt$ to the current data. 
% by pretending $\hat{q}_{yt}^z$ is the true data generating parameter.

\textbf{Greedy:} For each group $yt$, we approximate the expected distance 
from the currently estimated ATE to the new estimated ATE 
if we were to observe one additional sample from the group, 
and we do so by substituting the estimated $\hat{q}_{yt}^z$'s 
for the true data generating parameters (which we do not know).
%and treat it as an initial sample.
We then sample from the group for which the following quantity is the largest, %the furthermost away from the current estimated ATE
 i.e., the group that induces the largest expected change in the estimated ATE: 
 $$ \mathbb{E}\left[ \left|\widehat{\ATE}\left(q_{yt} = \frac{n_{yt}\hat{q}_{yt}+\mathrm{B}(\hat{q}_{yt})}{n_{yt}+1} \right) - \widehat{\ATE}(q_{yt}=\hat{q}_{yt}) \right| \right],$$
 where $\mathrm{B}(\hat{q}_{yt})$ denotes a Bernoulli variable 
 with mean $\hat{q}_{yt}$ (over which the expectation is taken), and 
%  abusing notation,
 $\widehat{\ATE}(q_{yt}=q)$ is the estimated $\ATE$ when 
 we update the estimate for $q_{yt}$ to $q$,
%  $q_{yt}$ is estimated as $q$ 
 and keep all other estimates unchanged.
 Intuitively, maximizing this quantity is meant as an approximate
 proxy for minimizing the expected distance between the estimated and true ATEs.


\textbf{$s$-Step Lookahead:} As a generalization of Greedy, 
which by definition looks one period ahead,
%of considering one additional sample at each time, 
we can consider policies that look $s$ samples ahead. 
More specifically, we consider all online policies over the next $s$ periods,
%group combinations that we can choose to sample in the next two steps and consider all possible data
%realizations.
%For each group combination, we then 
and calculate the expected distance from the currently 
estimated ATE to the estimated ATE $s$ periods from now.
%if we were to sample from those two groups.
Just as in Greedy, we choose the policy that maximizes this quantity,
%to sample from the first group of the combination that moves furthermost away from the current estimate.
%So, even though two steps
%are considered in our selection process,
%we only 
and implement the policy's first action. 
That is, we repeat the entire process at every period rather than every $s$ periods. 
The $s$-Step Lookahead policies should improve with increased $s$,
but this comes at a computational cost exponential in $s$.
% 
% (we average the new samples with the $\frac{1}{2}$)


% maintain a 
% Bayesian prior for each of unknown parameter $q_{yt}$, and estimate the uncertainty over ATE using the Monte Carlo sampling method.
% That is, we maintain $4$ beta distributions
% $\{B(\alpha_{yt}, \beta_{yt})\} %\coloneqq
% \triangleq \text{\textbf{B}}$
% for tracking our current posterior over each $q_{yt}$, where
% $(\alpha_{yt}, \beta_{yt})$ corresponds to the numbers 
% of observed occurrences of $Z=1$ and $Z=0$s, 
% respectively, for each group $yt$. 
% We initialize the beta prior with a uniform prior $(1, 1)$, 
% and the expected ATE
% is given as a function of $\bf a$ (known)
% and by marginalizing over the possible values of $\bf q$ 
% as described by our current beliefs \textbf{B}. 
% We denote this quantity $E_{\bf \hat{q} \sim \textbf{B}}[\text{ATE}(\bf a, \hat{q})]$, 
% and abbreviate it as $\widehat{\ATE}(\bf a, \textbf{B})$. 

% Similarly, we also formed a Bayesian priors when NSP, and OWSP were chosen. 
% Thus, the estimated ATE, $\hat{\text{ATE}}({{\bf a}, \text{\textbf{B}}}) = \int_{\text{\textbf{B}}} \text{ATE}({\bf a}, \beta) f_{\text{\textbf{B}}}(\beta) d\beta$, where $f_{\text{\textbf{B}}}(\beta)$ is the density function of \textbf{B}.

% \begin{enumerate}
    % \item \textbf{Online + only q} algorithm: 
    % \item \textbf{Naive (only \emph{q})}: 
    % In each iteration, the objective is to sample from category $i$ 
    % that gives the maximum expected reduction in the variance of $B_i$, denoted $Var(B_i)$. 
    % Let $B_i(0)$ and $B_i(1)$ be the posterior distributions for $q_i$ 
    % that would result from the events of sampling from group $i$
    % %  that we sample from category $i$
    % and observing $0$ and $1$, respectively. Furthermore, let $P(B_i(1))=E(B_i)$ denote the probability of drawing a $1$ from  $B_i$, and similarly, we define $P(B_i(1)) = 1-E(B_i)$.
    % % 
    % % Then, $Var(B_i(0))$ denotes the variance of $B_i$ 
    % % after updating it with a $0$, that is, $Var(B_i(0)) = Var(B_i(\alpha_i, \beta_i+1))$. 
    % % 
    % In the naive algorithm, we select an example to deconfound from group $i^*$ as given by
    % \begin{align*}
    % i^* = \argmax_{i\in\{4\}} &\left(Var(B_i)-Var(B_i(1))\right)
    % \cdot P(B_i(1))\\& +
    % \left(Var(B_i) - Var(B_i(0))\right)
    % \cdot P(B_i(0)). 
    % \end{align*}
    % Note that this algorithm is both naive (focusing on the parameters $q$ vs the ATE) and myopic,
    % focusing only on the next-turn reduction in uncertainty. 
    %  
    % Let $Var(B_i(0))$ denote the variance of $B_i$ 
    % after updating it with a $0$, that is, $Var(B_i(0)) = Var(B_i(\alpha_i, \beta_i+1))$. Thus, in each iteration, we would like to sample from category $i^* = \argmax_{i\in\{4\}} Var(B_i)-Var(B_i(1))\cdot P(B_i(1))-Var(B_i(0))\cdot P(B_i(0))$.
    % 
    % \paragraph{Selection Criterion}:
    % In each iteration, we simulate the reduction in uncertainty over ATE if we were to choose $yt$ to reveal the value for $Z$. We do so by drawing a $q_{yt}$ value from the posterior of $q_{yt}$, simulate the next data from Bernoulli$(q_{yt})$
    % , and use the simulated data to update the belief $B(\alpha_{yt}, \beta_{yt})$, and perform Monte Carlo sampling over this new posterior. And we repeat this process multiple times.
    % That is, let $\widehat{\ATE}({\bf a}, \textbf{B}_{yt}(1)) \coloneqq \widehat{\ATE}({\bf a}, B_{yt}(\alpha_{yt}+1, \beta_{yt}), B_{{\bar{yt}}\in\{00,01,10,11\}, \bar{yt}\neq {yt}}(\alpha_{\bar{yt}},\beta_{\bar{yt}}))$ be the estimated ATE if we choose to reveal the value for $q_{yt}$ in the next iteration and get 1. 
    % We define $\widehat{\text{ATE}}({\bf a}, \textbf{B}_{yt}(0))$ similarly. 
    % In each iteration, the objective is to sample from group $yt^* = \argmax_{yt\in\{00,01,10,11\}} |\widehat{\text{ATE}}({\bf a}, \textbf{B}_{yt}(1))-\widehat{\text{ATE}}({\bf a}, \textbf{B})|\cdot P(B_{yt}(1)) + |\widehat{\text{ATE}}({\bf a},\textbf{B}_{yt}(0))-\widehat{\text{ATE}}({\bf a}, \textbf{B})|\cdot P(B_{yt}(0)) + |\widehat{\text{ATE}}({\bf a}, \textbf{B}_{yt}(1))-\widehat{\text{ATE}}({\bf a},\textbf{B}_{yt}(0))|$.
    % Add: the interpretation of this objective function
    
\textbf{Synthetic Experiments }
As in the experiments in Section~\ref{sec:experiments}, 
Figure~\ref{fig:online} was generated using
1,300 instances sampled uniformly
from the unit $7$-Simplex,
and each instance contains $4$ replications.
The absolute error is measured as a function of the number of deconfounded samples 
in step sizes of $15$. 
    % For OSP, at each selection time stamp, to decide which group to sample the next data from, we sampled 2000 different $q_{yt}$ values from the posterior and calculated the average value of the objective function. Under all sample selection policies, to calculate the expected ATE from the posterior after a sampling decision has been made and data was revealed, 1000 sets of $q_{yt}$ were drawn from the posterior $\bf B$. 
    We observe that the
    % improvement of the 
    Greedy 
    and 2-Step Lookahead selection policies 
    outperform OWSP (Figure~\ref{fig:online}).
    Figure~\ref{fig:online} (middle, right) contain $50$ points, 
    each corresponding to one instance averaged over $1,000$ replications.
    The right scatter plot suggests that
    there are benefits of selecting sample online.
    However, the middle plot suggests 
    the improvement might be limited. 
    % \item \textbf{Online + Bayesian $q$ + MLE ATE} algorithm: in this version, we maintain and update the beta distribution over each q and select the next sample using the same criteria as the \textbf{online} algorithm. However, the estimated ATE is calculated using the frequency count, that is, the $\bf \hat{q}$ in estimated ATE, $\hat{\text{ATE}}(\bf a, \hat{q})$, is estimated by plugging in the MLE for $\bf q$, and $\bf a$ into the ATE function in Equation 1, where we initialize the value of $q_i$ to be $\frac{1}{2}$ if we do not have any observation for $q_i$ and as we get more data, we take the average of the $\frac{1}{2}$ and all observed data to get an estimated $q_i$. Let $n_i^0$ and $n_i^1$ denote the number of $0$ and $1$ that we have observed for each $q_i$ so far, and let $n_i$ be the total amount of data that we have observed for $q_i$, then the MLE for $q_i$, $\hat{q}_i = \frac{0.5 + n_i^1}{1+n_i}$.
    
    % \item \textbf{Online + pure MLE} algorithm: in this version, ATE is estimated using the same method as in \textbf{Online + Bayesian $q$ + MLE ATE} algorithm. However, we no longer maintain a beta distribution over each $q_i$ in the sample selection process. Let $\hat{\text{ATE}}({\bf a, \hat{q}_i(1)}):= \hat{\text{ATE}}({\bf a}, \hat{q}_i(1) :=\frac{n_i^1+1.5}{n_i + 2}, \hat{q}_{j\in\{4\},j\neq i})$, and similarly, $\hat{\text{ATE}}({\bf a, \hat{q}_i(0)}):= \hat{\text{ATE}}({\bf a}, \hat{q}_i(0) :=\frac{n_i^1+0.5}{n_i + 2}, \hat{q}_{j\in\{4\},j\neq i})$. 
    % Then, in the sample selection process, our objective is to sample from the category $i^* = \argmax_{i\in\{4\}} |\hat{\text{ATE}}({\bf a, \hat{q_i}(1)})-\hat{\text{ATE}}({\bf a, \hat{q}})|\cdot \hat{q}_i + |\hat{\text{ATE}}({\bf a,\hat{q_i}(0)})-\hat{\text{ATE}}({\bf a, \hat{q}})|\cdot (1-\hat{q}_i) + |\hat{\text{ATE}}({\bf a, \hat{q_i}(1)})-\hat{\text{ATE}}(\bf a,\hat{q_i}(0))|$.
    


    
    % \item \textbf{Online + lower bound} algorithm: to create our lower bound, in this version, we sample from all 4 categories in each step. 
    % %(improved version: we group the horizons into multiples of 4. In the first period, we sample from category 1,2,3; in the second, 2,3,4; in the third, 3,4,1; in the fourth, 4,1,2. Thus, in every 4 periods, we are guaranteed that we sample from each data category exactly 3 times. The only possible way that the optimal solution is better than this sampling policy is when it is optimal to sample from all 4 data from the same category more than $\frac{3}{4}T$ times, where $T$ is the length of total horizon. We can either show that this ${\bf a,q}$ happens with very small probability or this contradicts some inherent property of our estimation problem.)
% \end{enumerate}

==> sections/proofcopy.tex <==
\begin{proof}[Proof of Theorem~\ref{thm:general_lower}]

We will proceed by construction. Consider ${\bf q} = (q_{00}, q_{01}, \beta, \beta+\gamma)$ and ${\bf q}' = (q_{00}, q_{01}, \beta+ \gamma, \beta )$, with $\beta, \beta+\gamma \in[\eta, 1-\eta]$. Then
\begin{align*}
&\ATE_{\bf a}({\bf q}) = 
\frac{a_{11}(\beta+\gamma)}{a_{11}(\beta+\gamma) + a_{01}q_{01}}
(a_{00}q_{00} + a_{01}q_{01} + a_{10}\beta+ a_{11}(\beta+\gamma)) 
+ \\&\frac{a_{11}(1-\beta-\gamma)}{a_{11}(1-\beta-\gamma) + a_{01}(1-q_{01})}
(1- a_{00}q_{00} - a_{01}q_{01} - a_{10}\beta 
- a_{11}(\beta+\gamma)) 
-\\&
\frac{a_{10}\beta}{a_{10}\beta+a_{00}q_{00}}(a_{00}q_{00} + a_{01}q_{01} + a_{10}\beta+ a_{11}(\beta+\gamma))
-
\\& \frac{a_{10}(1-\beta)}{a_{10}(1-\beta)+a_{00}(1-q_{00})}(1- a_{00}q_{00} - a_{01}q_{01} - a_{10}\beta 
- a_{11}(\beta+\gamma)) ,
\end{align*}
and similarly, we have
\begin{align*}
&\ATE_{\bf a}({\bf q}') =
\frac{a_{11}\beta}{a_{11}\beta + a_{01}q_{01}}
(a_{00}q_{00} + a_{01}q_{01} + a_{10}(\beta+\gamma)+ a_{11}\beta) +
\\&
\frac{a_{11}(1-\beta)}{a_{11}(1-\beta) + a_{01}(1-q_{01})}(1- a_{00}q_{00} - a_{01}q_{01} - a_{10}(\beta+\gamma)
- a_{11}\beta 
) -
\\&
\frac{a_{10}(\beta+\gamma)}{a_{10}(\beta+\gamma)+a_{00}q_{00}}(a_{00}q_{00} + a_{01}q_{01} + a_{10}(\beta+\gamma)+ a_{11}\beta) - 
\\&
\frac{a_{10}(1-\beta-\gamma)}{a_{10}(1-\beta-\gamma)+a_{00}(1-q_{00})}(1- a_{00}q_{00} - a_{01}q_{01} - a_{10}(\beta+\gamma)
- a_{11}\beta
).
\end{align*}
Ignoring the $\gamma$ in the denominator, we have that 
\begin{align}
&\ATE_{\bf a}({\bf q})-\ATE_{\bf a}({\bf q}') =
(\frac{a_{11}}{a_{11}\beta+a_{01}q_{01}}+\frac{a_{10}}{a_{10}\beta+a_{00}q_{00}})(a_{00}q_{00}+a_{01}q_{01}+a_{10}\beta+a_{11}\beta)\gamma \nonumber
\\& 
-(\frac{a_{11}}{a_{11}(1-\beta)+a_{01}(1-q_{01})}+\frac{a_{10}}{a_{10}(1-\beta)+a_{00}(1-q_{00})})(1-a_{00}q_{00}-a_{01}q_{01}-a_{10}\beta-a_{11}\beta)\gamma \nonumber
\\& 
+\frac{a_{11}^2-a_{11}a_{10}}{a_{11}\beta+a_{01}q_{01}}\beta\gamma - \frac{a_{11}^2-a_{11}a_{10}}{a_{11}(1-\beta)+a_{01}(1-q_{01})}(1-\beta)\gamma \nonumber
\\&
+\frac{a_{10}^2-a_{11}a_{10}}{a_{10}\beta+a_{00}q_{00}}\beta\gamma - \frac{a_{10}^2-a_{11}a_{10}}{a_{10}(1-\beta)+a_{00}(1-q_{00})}(1-\beta)\gamma \nonumber
\\&
+ \frac{a_{11}^2}{a_{11}\beta+a_{01}q_{01}}\gamma^2 + \frac{a_{11}^2}{a_{11}(1-\beta)+a_{01}(1-q_{01})}\gamma^2 \nonumber
\\&
+ \frac{a_{10}^2}{a_{10}\beta+a_{00}q_{00}}\gamma^2 + \frac{a_{10}^2}{a_{10}(1-\beta)+a_{00}(1-q_{00})}\gamma^2 \label{eq:ATE_diff}
\end{align}

Similar to the proof above, let $B_1$ denote the Bernoulli random variable with parameter $\beta$, and let $B_2$ denote the Bernoulli random variable with parameter $\beta+\gamma$. Then, given $m$ deconfounded samples, we have $\mathrm{KL}(B_1^m\|B_2^m) \leq m\beta\log(\frac{\beta}{\beta+\gamma}) + m(1-\beta)\log(\frac{1-\beta}{1-\beta-\gamma})\leq m\log(1+\frac{\gamma}{1-\beta-\gamma}) \leq m(\frac{\gamma}{1-\beta-\gamma} - \frac{\gamma^2}{2(1-\beta-\gamma)^2}) $. Thus, we have $m\sim \Omega(\frac{\log(\delta^{-1})}{\gamma^2})$. From Equation (\ref{eq:ATE_diff}), we observe that $\epsilon = \|\ATE_{\bf a}({\bf q}) - \ATE_{\bf a}({\bf q}')\| \sim \Omega (\gamma)$. Combining above, we have $m\sim \Omega(\frac{\log(\delta^{-1})}{\epsilon^2})$.

Now ignoring the terms that are in $\gamma^2$, Equation (\ref{eq:ATE_diff}) is
\begin{align*}
&\approx \Bigg[(\frac{a_{11}}{a_{11}\beta+a_{01}q_{01}}+\frac{a_{10}}{a_{10}\beta+a_{00}q_{00}})(a_{00}q_{00}+a_{01}q_{01}) +\frac{2a_{11}^2\beta}{a_{11}\beta+a_{01}q_{01}} + \frac{2a_{10}^2\beta}{a_{10}\beta+a_{00}q_{00}}
\\& 
-(\frac{a_{11}}{a_{11}(1-\beta)+a_{01}(1-q_{01})}+\frac{a_{10}}{a_{10}(1-\beta)+a_{00}(1-q_{00})})(a_{00}(1-q_{00})+a_{01}(1-q_{01}))
\\&
-\frac{2a_{11}^2(1-\beta)}{a_{11}(1-\beta)+a_{01}(1-q_{01})}-\frac{2a_{10}^2(1-\beta)}{a_{10}(1-\beta)+a_{00}(1-q_{00})} \Bigg]\gamma
% \\& 
% + \frac{a_{11}^2}{a_{11}\beta+a_{01}q_{01}}\gamma^2 - \frac{a_{11}^2}{a_{11}(1-\beta)+a_{01}(1-q_{01})}\gamma^2
% \\&
% + \frac{a_{10}^2}{a_{10}\beta+a_{00}q_{00}}\gamma^2 - \frac{a_{10}^2}{a_{10}(1-\beta)+a_{00}(1-q_{00})}\gamma^2
\end{align*}

The 
%minimum
maximum
of the above equation is achieved at 
either $q_{00} = \beta$ and $q_{01} = 1-\beta$, or $q_{00} = 1-\beta$ and $q_{01} = \beta$.
Thus, the maximum of the coefficient in front of $\gamma$ equals to
\begin{align*}
    \max\mathrm{abs}\Big(&\frac{a_{11}a_{00}(1-2\beta)}{(a_{11}+a_{01})(1-\beta)\beta}-\frac{2a_{10}^3a_{00}(1-2\beta)}{(a_{10}(1-\beta)+a_{00}\beta)(a_{10}\beta+a_{00}(1-\beta))},\\&
    \frac{a_{10}a_{00}(1-2\beta)}{(a_{10}+a_{00})(1-\beta)\beta}-\frac{2a_{11}^3a_{01}(1-2\beta)}{(a_{11}(1-\beta)+a_{01}\beta)(a_{11}\beta+a_{01}(1-\beta))}\Big) 
\end{align*}

% $q_{00} = q_{01} = \beta$ with the coefficient in front of $\gamma$ to be $=0$. This left us with the second order terms in $\gamma^2$ with the coefficient equals to
% $$(\frac{1}{\beta}+\frac{1}{1-\beta})(\frac{a_{11}^2}{a_{11}+a_{01}}+\frac{a_{10}^2}{a_{10}+a_{00}}).$$


Consider ${\bf q} = (q_{00}, \beta, q_{10}, \beta+\gamma)$ and ${\bf q}' = (q_{00},  \beta+ \gamma, q_{10}, \beta )$, with $\beta, \beta+\gamma \in[\eta, 1-\eta]$. Then,
\begin{align*}
&\ATE_{\bf a}({\bf q}) = 
\frac{a_{11}(\beta+\gamma)}{a_{11}(\beta+\gamma) + a_{01}\beta}
(a_{00}q_{00} + a_{01}\beta + a_{10}q_{10}+ a_{11}(\beta+\gamma)) 
+ \\&\frac{a_{11}(1-\beta-\gamma)}{a_{11}(1-\beta-\gamma) + a_{01}(1-\beta)}
(1- a_{00}q_{00} - a_{01}\beta - a_{10}q_{10} 
- a_{11}(\beta+\gamma)) 
-\\&
\frac{a_{10}q_{10}}{a_{10}q_{10}+a_{00}q_{00}}(a_{00}q_{00} + a_{01}\beta + a_{10}q_{10}+ a_{11}(\beta+\gamma))
-
\\& \frac{a_{10}(1-q_{10})}{a_{10}(1-q_{10})+a_{00}(1-q_{00})}(1- a_{00}q_{00} - a_{01}\beta - a_{10}q_{10}
- a_{11}(\beta+\gamma)) ,
\end{align*}
and similarly, we have
\begin{align*}
&\ATE_{\bf a}({\bf q}') =
\frac{a_{11}\beta}{a_{11}\beta + a_{01}(\beta+\gamma)}
(a_{00}q_{00} + a_{01}(\beta+\gamma) + a_{10}q_{10}+ a_{11}\beta) +
\\&
\frac{a_{11}(1-\beta)}{a_{11}(1-\beta) + a_{01}(1-\beta-\gamma)}(1- a_{00}q_{00} - a_{01}(\beta+\gamma) - a_{10}q_{10}
- a_{11}\beta 
) -
\\&
\frac{a_{10}q_{10}}{a_{10}q_{10}+a_{00}q_{00}}(a_{00}q_{00} + a_{01}(\beta+\gamma) + a_{10}q_{10}+ a_{11}\beta) - 
\\&
\frac{a_{10}(1-q_{10})}{a_{10}(1-q_{10})+a_{00}(1-q_{00})}(1- a_{00}q_{00} - a_{01}(\beta+\gamma) - a_{10}q_{10}
- a_{11}\beta
).
\end{align*}
Ignoring the $\gamma$ in the denominator, we have that 
\begin{align}
&\ATE_{\bf a}({\bf q})-\ATE_{\bf a}({\bf q}') 
=
(\frac{a_{11}}{a_{11}\beta+a_{01}\beta}
%+\frac{a_{10}}{a_{10}q_{10}+a_{00}q_{00}}
)(a_{00}q_{00}+a_{01}\beta+a_{10}q_{10}+a_{11}\beta)\gamma \nonumber
\\& 
-(\frac{a_{11}}{a_{11}(1-\beta)+a_{01}(1-\beta)}
%+\frac{a_{10}}{a_{10}(1-q_{10})+a_{00}(1-q_{00})}
)(1-a_{00}q_{00}-a_{01}\beta-a_{10}q_{10}-a_{11}\beta)\gamma \nonumber
%\\& 
%+\frac{a_{11}^2-a_{11}a_{10}}{a_{11}\beta+a_{01}\beta}\gamma - \frac{a_{11}^2-a_{11}a_{10}}{a_{11}(1-\beta)+a_{01}(1-\beta)}(1-\beta)\gamma \nonumber
\\&
+\frac{a_{10}q_{10}(a_{01}-a_{11})}{a_{10}q_{10}+a_{00}q_{00}}\gamma - \frac{a_{10}(1-q_{10})(a_{01}-a_{11})}{a_{10}(1-q_{10})+a_{00}(1-q_{00})}\gamma \nonumber
\\&
+ \frac{a_{11}^2}{a_{11}\beta+a_{01}\beta}\gamma^2 + \frac{a_{11}^2}{a_{11}(1-\beta)+a_{01}(1-\beta)}\gamma^2  \label{eq:ATE_diff2}
\end{align}
Similarly, when $q_{00} = q_{10} =1-\beta$, the coefficient in front of $\gamma$ is
$$a_{11} + \frac{a_{11}}{a_{11}+a_{01}}(\frac{1}{\beta}-\frac{1-(a_{01}+a_{11})\beta}{1-\beta}).$$

Observe that 
the largest coefficient in front of $\gamma$ achieves in this case. Note that this is also equivalent to having the highest lower bound. In this particular case, $\epsilon\approx \frac{a_{11}}{a_{11}+a_{01}}\frac{1}{\beta}\gamma$, thus, the number of deconfounded samples needed is approximately $$m\sim C_1 \frac{\log(\delta^{-1})a_{11}^2}{\epsilon^2 (a_{11}+a_{01})^2\beta^2}.$$

Thus under natural selection policy, we need at least $\frac{m}{a_{11}}$ samples; uniform selection policy, we need at least $4m$ deconfounded samples; under outcome-weighted selection policy, we need at least $2\frac{a_{11}+a_{01}}{a_{11}}m$ deconfounded samples.


%becomes zero, and we are left with the second order term, where the coefficient in front of $\gamma^2$ is
% $$(\frac{1}{\beta}+\frac{1}{1-\beta})\frac{a_{11}^2}{a_{11}+a_{01}}.$$

Consider ${\bf q} = (\beta, q_{01}, q_{10}, \beta+\gamma)$ and ${\bf q}' = (\beta+ \gamma, q_{01}, q_{10}, \beta )$, with $\beta, \beta+\gamma \in[\eta, 1-\eta]$. Then,
\begin{align*}
&\ATE_{\bf a}({\bf q}) = 
\frac{a_{11}(\beta+\gamma)}{a_{11}(\beta+\gamma) + a_{01}q_{01}}
(a_{00}\beta + a_{01}q_{01} + a_{10}q_{10}+ a_{11}(\beta+\gamma)) 
+ \\&\frac{a_{11}(1-\beta-\gamma)}{a_{11}(1-\beta-\gamma) + a_{01}(1-q_{01})}
(1- a_{00}\beta - a_{01}q_{01} - a_{10}q_{10} 
- a_{11}(\beta+\gamma)) 
-\\&
\frac{a_{10}q_{10}}{a_{10}q_{10}+a_{00}\beta}(a_{00}\beta + a_{01}q_{01} + a_{10}q_{10}+ a_{11}(\beta+\gamma))
-
\\& \frac{a_{10}(1-q_{10})}{a_{10}(1-q_{10})+a_{00}(1-q_{00})}(1- a_{00}\beta - a_{01}q_{01} - a_{10}q_{10}
- a_{11}(\beta+\gamma)) ,
\end{align*}
and similarly, we have
\begin{align*}
&\ATE_{\bf a}({\bf q}') =
\frac{a_{11}\beta}{a_{11}\beta + a_{01}q_{01}}
(a_{00}(\beta+\gamma) + a_{01}q_{01} + a_{10}q_{10}+ a_{11}\beta) +
\\&
\frac{a_{11}(1-\beta)}{a_{11}(1-\beta) + a_{01}(1-q_{01})}(1- a_{00}(\beta+\gamma) - a_{01}q_{01} - a_{10}q_{10}
- a_{11}\beta 
) -
\\&
\frac{a_{10}q_{10}}{a_{10}q_{10}+a_{00}(\beta+\gamma)}(a_{00}(\beta+\gamma) + a_{01}q_{01} + a_{10}q_{10}+ a_{11}\beta) - 
\\&
\frac{a_{10}(1-q_{10})}{a_{10}(1-q_{10})+a_{00}(1-\beta-\gamma)}(1- a_{00}(\beta+\gamma) - a_{01}q_{01} - a_{10}q_{10}
- a_{11}\beta
).
\end{align*}

Ignoring the $\gamma$ in the denominator, we have that 
\begin{align}
&\ATE_{\bf a}({\bf q})-\ATE_{\bf a}({\bf q}') =
(\frac{a_{11}}{a_{11}\beta+a_{01}q_{01}}
%+\frac{a_{10}}{a_{10}\beta+a_{00}q_{00}}
)
(a_{00}\beta+a_{01}q_{01}+a_{10}q_{10}+a_{11}\beta)\gamma \nonumber
\\& 
-(\frac{a_{11}}{a_{11}(1-\beta)+a_{01}(1-q_{01})}
%+\frac{a_{10}}{a_{10}(1-\beta)+a_{00}(1-q_{00})}
)(1-a_{00}\beta-a_{01}q_{01}-a_{10}q_{10}-a_{11}\beta)\gamma \nonumber
\\& 
+\frac{a_{11}^2-a_{11}a_{10}}{a_{11}\beta+a_{01}q_{01}}\beta\gamma - \frac{a_{11}^2-a_{11}a_{10}}{a_{11}(1-\beta)+a_{01}(1-q_{01})}(1-\beta)\gamma \nonumber
\\&
+\frac{a_{10}q_{10}(a_{00}-a_{11})}{a_{10}q_{10}+a_{00}\beta}\gamma - \frac{a_{10}(1-q_{10})(a_{00}-a_{11})}{a_{10}(1-q_{10})+a_{00}(1-\beta)}\gamma \nonumber
\\&
+ \frac{a_{11}^2}{a_{11}\beta+a_{01}q_{01}}\gamma^2 + \frac{a_{11}^2}{a_{11}(1-\beta)+a_{01}(1-q_{01})}\gamma^2 \label{eq:ATE_diff3}
\end{align}
The maximum is achieved at $q_{01}=\beta, q_{10}=1-\beta$. The coefficient is
$$\frac{a_{11}a_{10}(1-2\beta)}{(a_{11}+a_{01})\beta(1-\beta)}+\frac{a_{10}(a_{00}-a_{11})a_{00}(1-2\beta)}{(a_{10}(1-\beta)+a_{00}\beta)(a_{10}\beta+a_{00}(1-\beta))}.$$
\end{proof}
